Integral equation method for the 1D steady-state Poisson-Nernst-Planck equations

An integral equation method is presented for the 1D steady-state Poisson-Nernst-Planck equations modeling ion transport through membrane channels. The differential equations are recast as integral equations using Green's 3rd identity yielding a fixed-point problem for the electric potential gradient and ion concentrations. The integrals are discretized by a combination of midpoint and trapezoid rules and the resulting algebraic equations are solved by Gummel iteration. Numerical tests for electroneutral and non-electroneutral systems demonstrate the method's 2nd order accuracy and ability to resolve sharp boundary layers. The method is applied to a 1D model of the K$^+$ ion channel with a fixed charge density that ensures cation selectivity. In these tests, the proposed integral equation method yields potential and concentration profiles in good agreement with published results.

==> notes_PNP.tex <==
for revision
- add middle initial "S" to Eisenberg in ref[20]
- name for $\phi_\pm$

other
- watch K+ ion channel video
